Quantum Search for Scaled Hash Function Preimages

We present the implementation of Grover's algorithm in a quantum simulator to perform a quantum search for preimages of two scaled hash functions, whose design only uses modular addition, word rotation, and bitwise exclusive or. Our implementation provides the means to assess with precision the scaling of the number of gates and depth of a full-fledged quantum circuit designed to find the preimages of a given hash digest. The detailed construction of the quantum oracle shows that the presence of AND gates, OR gates, shifts of bits and the reuse of the initial state along the computation, require extra quantum resources as compared with other hash functions based on modular additions, XOR gates and rotations. We also track the entanglement entropy present in the quantum register at every step along the computation, showing that it becomes maximal at the inner core of the first action of the quantum oracle, which implies that no classical simulation based on Tensor Networks would be of relevance. Finally, we show that strategies that suggest a shortcut based on sampling the quantum register after a few steps of Grover's algorithm can only provide some marginal practical advantage in terms of error mitigation.

==> figures/blake2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,162); %set diagram left start at 0, and has height of 162

%Shape: Grid [id:dp4389325023573263] 
\draw  [draw opacity=0] (199.67,30) -- (240,30) -- (240,70.17) -- (199.67,70.17) -- cycle ; \draw   (199.67,30) -- (199.67,70.17)(209.67,30) -- (209.67,70.17)(219.67,30) -- (219.67,70.17)(229.67,30) -- (229.67,70.17)(239.67,30) -- (239.67,70.17) ; \draw   (199.67,30) -- (240,30)(199.67,40) -- (240,40)(199.67,50) -- (240,50)(199.67,60) -- (240,60)(199.67,70) -- (240,70) ; \draw    ;
%Shape: Grid [id:dp7504086232861402] 
\draw  [draw opacity=0] (140,99.83) -- (180.67,99.83) -- (180.67,120) -- (140,120) -- cycle ; \draw   (140,99.83) -- (140,120)(150,99.83) -- (150,120)(160,99.83) -- (160,120)(170,99.83) -- (170,120)(180,99.83) -- (180,120) ; \draw   (140,99.83) -- (180.67,99.83)(140,109.83) -- (180.67,109.83)(140,119.83) -- (180.67,119.83) ; \draw    ;
%Rounded Rect [id:dp5112290593462414] 
\draw   (200,98) .. controls (200,93.58) and (203.58,90) .. (208,90) -- (232,90) .. controls (236.42,90) and (240,93.58) .. (240,98) -- (240,122) .. controls (240,126.42) and (236.42,130) .. (232,130) -- (208,130) .. controls (203.58,130) and (200,126.42) .. (200,122) -- cycle ;
%Straight Lines [id:da5002180687945932] 
\draw    (180,109.83) -- (198,109.98) ;
\draw [shift={(200,110)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2922131158990813] 
\draw    (240,110) -- (258,110.15) ;
\draw [shift={(260,110.17)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da06399498629921219] 
\draw    (219.67,70) -- (219.97,88) ;
\draw [shift={(220,90)}, rotate = 269.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp7735553517269926] 
\draw  [draw opacity=0] (319.67,30) -- (360,30) -- (360,70.17) -- (319.67,70.17) -- cycle ; \draw   (319.67,30) -- (319.67,70.17)(329.67,30) -- (329.67,70.17)(339.67,30) -- (339.67,70.17)(349.67,30) -- (349.67,70.17)(359.67,30) -- (359.67,70.17) ; \draw   (319.67,30) -- (360,30)(319.67,40) -- (360,40)(319.67,50) -- (360,50)(319.67,60) -- (360,60)(319.67,70) -- (360,70) ; \draw    ;
%Shape: Grid [id:dp5837977244917669] 
\draw  [draw opacity=0] (260,99.83) -- (300.67,99.83) -- (300.67,120) -- (260,120) -- cycle ; \draw   (260,99.83) -- (260,120)(270,99.83) -- (270,120)(280,99.83) -- (280,120)(290,99.83) -- (290,120)(300,99.83) -- (300,120) ; \draw   (260,99.83) -- (300.67,99.83)(260,109.83) -- (300.67,109.83)(260,119.83) -- (300.67,119.83) ; \draw    ;
%Rounded Rect [id:dp16048985458025422] 
\draw   (320,98) .. controls (320,93.58) and (323.58,90) .. (328,90) -- (352,90) .. controls (356.42,90) and (360,93.58) .. (360,98) -- (360,122) .. controls (360,126.42) and (356.42,130) .. (352,130) -- (328,130) .. controls (323.58,130) and (320,126.42) .. (320,122) -- cycle ;
%Straight Lines [id:da7853971074392705] 
\draw    (300,109.83) -- (318,109.98) ;
\draw [shift={(320,110)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4099666517758407] 
\draw    (360,110) -- (378,110.15) ;
\draw [shift={(380,110.17)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1903233012509149] 
\draw    (339.67,70) -- (339.97,88) ;
\draw [shift={(340,90)}, rotate = 269.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp8925841733778084] 
\draw  [draw opacity=0] (479.67,30) -- (520,30) -- (520,70.17) -- (479.67,70.17) -- cycle ; \draw   (479.67,30) -- (479.67,70.17)(489.67,30) -- (489.67,70.17)(499.67,30) -- (499.67,70.17)(509.67,30) -- (509.67,70.17)(519.67,30) -- (519.67,70.17) ; \draw   (479.67,30) -- (520,30)(479.67,40) -- (520,40)(479.67,50) -- (520,50)(479.67,60) -- (520,60)(479.67,70) -- (520,70) ; \draw    ;
%Shape: Grid [id:dp7677580195936737] 
\draw  [draw opacity=0] (420,99.83) -- (460.67,99.83) -- (460.67,120) -- (420,120) -- cycle ; \draw   (420,99.83) -- (420,120)(430,99.83) -- (430,120)(440,99.83) -- (440,120)(450,99.83) -- (450,120)(460,99.83) -- (460,120) ; \draw   (420,99.83) -- (460.67,99.83)(420,109.83) -- (460.67,109.83)(420,119.83) -- (460.67,119.83) ; \draw    ;
%Rounded Rect [id:dp16998303474927545] 
\draw   (480,98) .. controls (480,93.58) and (483.58,90) .. (488,90) -- (512,90) .. controls (516.42,90) and (520,93.58) .. (520,98) -- (520,122) .. controls (520,126.42) and (516.42,130) .. (512,130) -- (488,130) .. controls (483.58,130) and (480,126.42) .. (480,122) -- cycle ;
%Straight Lines [id:da911105039619668] 
\draw    (460,109.83) -- (478,109.98) ;
\draw [shift={(480,110)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4717099342882849] 
\draw    (520,110) -- (538,110.15) ;
\draw [shift={(540,110.17)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da09656733706514253] 
\draw    (499.67,70) -- (499.97,88) ;
\draw [shift={(500,90)}, rotate = 269.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6357671929159483] 
\draw    (400,109.67) -- (418,109.82) ;
\draw [shift={(420,109.83)}, rotate = 180.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp5890767782491497] 
\draw  [draw opacity=0] (540,100.17) -- (580.67,100.17) -- (580.67,120.33) -- (540,120.33) -- cycle ; \draw   (540,100.17) -- (540,120.33)(550,100.17) -- (550,120.33)(560,100.17) -- (560,120.33)(570,100.17) -- (570,120.33)(580,100.17) -- (580,120.33) ; \draw   (540,100.17) -- (580.67,100.17)(540,110.17) -- (580.67,110.17)(540,120.17) -- (580.67,120.17) ; \draw    ;
%Straight Lines [id:da160895717067028] 
\draw    (160,119.83) -- (160,150) ;
%Straight Lines [id:da6780590850154404] 
\draw    (160,150) -- (500,150) ;
%Straight Lines [id:da19641090987468757] 
\draw    (220,150) -- (220,132) ;
\draw [shift={(220,130)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da03053460246748485] 
\draw    (340,150) -- (340,132) ;
\draw [shift={(340,130)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10985069107503298] 
\draw    (500,150) -- (500,132) ;
\draw [shift={(500,130)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (214,101.4) node [anchor=north west][inner sep=0.75pt]    {$F$};
% Text Node
\draw (154,82.4) node [anchor=north west][inner sep=0.75pt]    {$iv$};
% Text Node
\draw (212,10.4) node [anchor=north west][inner sep=0.75pt]    {$d_{0}$};
% Text Node
\draw (334,101.4) node [anchor=north west][inner sep=0.75pt]    {$F$};
% Text Node
\draw (275,82.4) node [anchor=north west][inner sep=0.75pt]    {$h$};
% Text Node
\draw (332,10.4) node [anchor=north west][inner sep=0.75pt]    {$d_{1}$};
% Text Node
\draw (494,101.4) node [anchor=north west][inner sep=0.75pt]    {$F$};
% Text Node
\draw (435,82.4) node [anchor=north west][inner sep=0.75pt]    {$h$};
% Text Node
\draw (482,10.4) node [anchor=north west][inner sep=0.75pt]    {$d_{n-1}$};
% Text Node
\draw (376,101.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots $};
% Text Node
\draw (555,82.4) node [anchor=north west][inner sep=0.75pt]    {$h$};


\end{tikzpicture}


==> figures/blake2_compression_function.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,181); %set diagram left start at 0, and has height of 181

%Shape: Grid [id:dp45143938957410756] 
\draw  [draw opacity=0] (80.86,19.5) -- (121.14,19.5) -- (121.14,59.79) -- (80.86,59.79) -- cycle ; \draw   (80.86,19.5) -- (80.86,59.79)(90.86,19.5) -- (90.86,59.79)(100.86,19.5) -- (100.86,59.79)(110.86,19.5) -- (110.86,59.79)(120.86,19.5) -- (120.86,59.79) ; \draw   (80.86,19.5) -- (121.14,19.5)(80.86,29.5) -- (121.14,29.5)(80.86,39.5) -- (121.14,39.5)(80.86,49.5) -- (121.14,49.5)(80.86,59.5) -- (121.14,59.5) ; \draw    ;
%Shape: Grid [id:dp5817677907729863] 
\draw  [draw opacity=0] (80.43,110.43) -- (120.57,110.43) -- (120.57,130.79) -- (80.43,130.79) -- cycle ; \draw   (80.43,110.43) -- (80.43,130.79)(90.43,110.43) -- (90.43,130.79)(100.43,110.43) -- (100.43,130.79)(110.43,110.43) -- (110.43,130.79)(120.43,110.43) -- (120.43,130.79) ; \draw   (80.43,110.43) -- (120.57,110.43)(80.43,120.43) -- (120.57,120.43)(80.43,130.43) -- (120.57,130.43) ; \draw    ;
%Rounded Rect [id:dp13847553636834253] 
\draw   (157.43,107.86) .. controls (157.43,103.44) and (161.01,99.86) .. (165.43,99.86) -- (190.14,99.86) .. controls (194.56,99.86) and (198.14,103.44) .. (198.14,107.86) -- (198.14,131.86) .. controls (198.14,136.28) and (194.56,139.86) .. (190.14,139.86) -- (165.43,139.86) .. controls (161.01,139.86) and (157.43,136.28) .. (157.43,131.86) -- cycle ;
%Shape: Grid [id:dp10978687687749189] 
\draw  [draw opacity=0] (217.86,100.21) -- (258.14,100.21) -- (258.14,140.5) -- (217.86,140.5) -- cycle ; \draw   (217.86,100.21) -- (217.86,140.5)(227.86,100.21) -- (227.86,140.5)(237.86,100.21) -- (237.86,140.5)(247.86,100.21) -- (247.86,140.5)(257.86,100.21) -- (257.86,140.5) ; \draw   (217.86,100.21) -- (258.14,100.21)(217.86,110.21) -- (258.14,110.21)(217.86,120.21) -- (258.14,120.21)(217.86,130.21) -- (258.14,130.21)(217.86,140.21) -- (258.14,140.21) ; \draw    ;
%Rounded Rect [id:dp21134492046321407] 
\draw   (278,108.71) .. controls (278,104.3) and (281.58,100.71) .. (286,100.71) -- (310.71,100.71) .. controls (315.13,100.71) and (318.71,104.3) .. (318.71,108.71) -- (318.71,132.71) .. controls (318.71,137.13) and (315.13,140.71) .. (310.71,140.71) -- (286,140.71) .. controls (281.58,140.71) and (278,137.13) .. (278,132.71) -- cycle ;
%Straight Lines [id:da122616355634112] 
\draw    (198.43,119.93) -- (215.86,120.18) ;
\draw [shift={(217.86,120.21)}, rotate = 180.84] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da17785224647711106] 
\draw    (257.86,120.21) -- (275.29,120.47) ;
\draw [shift={(277.29,120.5)}, rotate = 180.84] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp01522655149114005] 
\draw  [draw opacity=0] (338.43,99.93) -- (378.71,99.93) -- (378.71,140.21) -- (338.43,140.21) -- cycle ; \draw   (338.43,99.93) -- (338.43,140.21)(348.43,99.93) -- (348.43,140.21)(358.43,99.93) -- (358.43,140.21)(368.43,99.93) -- (368.43,140.21)(378.43,99.93) -- (378.43,140.21) ; \draw   (338.43,99.93) -- (378.71,99.93)(338.43,109.93) -- (378.71,109.93)(338.43,119.93) -- (378.71,119.93)(338.43,129.93) -- (378.71,129.93)(338.43,139.93) -- (378.71,139.93) ; \draw    ;
%Rounded Rect [id:dp4396478253838745] 
\draw   (397.57,108.43) .. controls (397.57,104.01) and (401.15,100.43) .. (405.57,100.43) -- (430.29,100.43) .. controls (434.7,100.43) and (438.29,104.01) .. (438.29,108.43) -- (438.29,132.43) .. controls (438.29,136.85) and (434.7,140.43) .. (430.29,140.43) -- (405.57,140.43) .. controls (401.15,140.43) and (397.57,136.85) .. (397.57,132.43) -- cycle ;
%Straight Lines [id:da25671452500507264] 
\draw    (319,119.64) -- (336.43,119.9) ;
\draw [shift={(338.43,119.93)}, rotate = 180.84] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7667251776379722] 
\draw    (378.43,119.93) -- (395.86,120.18) ;
\draw [shift={(397.86,120.21)}, rotate = 180.84] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da14223627846747577] 
\draw    (120.43,120.43) -- (154.86,120.7) ;
\draw [shift={(156.86,120.71)}, rotate = 180.45] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4244746484678157] 
\draw    (438.86,120.21) -- (475.86,120.21) ;
\draw [shift={(477.86,120.21)}, rotate = 540] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da640124671717488] - output DiagQR going down
\draw    (458,150) -- (458,120.21) ;
%Straight Lines [id:da9294367179415881] - i=0..rho-1 line
\draw    (204,150) -- (458,150) ;
%Straight Lines [id:da28966806125798095] - line going back to init
\draw    (204,150) -- (204,122) ;
\draw [shift={(204,122)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Grid [id:dp06431415207717572] 
\draw  [draw opacity=0] (477.86,98.21) -- (518,98.21) -- (518,118.57) -- (477.86,118.57) -- cycle ; \draw   (477.86,98.21) -- (477.86,118.57)(487.86,98.21) -- (487.86,118.57)(497.86,98.21) -- (497.86,118.57)(507.86,98.21) -- (507.86,118.57)(517.86,98.21) -- (517.86,118.57) ; \draw   (477.86,98.21) -- (518,98.21)(477.86,108.21) -- (518,108.21)(477.86,118.21) -- (518,118.21) ; \draw    ;
%Shape: Grid [id:dp8844535100862108] 
\draw  [draw opacity=0] (477.86,121.79) -- (518,121.79) -- (518,142.14) -- (477.86,142.14) -- cycle ; \draw   (477.86,121.79) -- (477.86,142.14)(487.86,121.79) -- (487.86,142.14)(497.86,121.79) -- (497.86,142.14)(507.86,121.79) -- (507.86,142.14)(517.86,121.79) -- (517.86,142.14) ; \draw   (477.86,121.79) -- (518,121.79)(477.86,131.79) -- (518,131.79)(477.86,141.79) -- (518,141.79) ; \draw    ;
\draw   (538.43,120.21) .. controls (538.43,114.69) and (542.91,110.21) .. (548.43,110.21) .. controls (553.95,110.21) and (558.43,114.69) .. (558.43,120.21) .. controls (558.43,125.74) and (553.95,130.21) .. (548.43,130.21) .. controls (542.91,130.21) and (538.43,125.74) .. (538.43,120.21) -- cycle ; \draw   (538.43,120.21) -- (558.43,120.21) ; \draw   (548.43,110.21) -- (548.43,130.21) ;
%Straight Lines [id:da4626181148044344] 
\draw    (140.57,120.71) -- (140.86,159.93) ;
%Straight Lines [id:da4235153159721301] 
\draw    (140.86,159.93) -- (547.86,160.21) ;
%Straight Lines [id:da5812638481632679] 
\draw    (547.86,160.21) -- (548.39,132.5) ;
\draw [shift={(548.43,130.5)}, rotate = 451.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da02697134965827286] 
\draw    (517.86,131.79) -- (536.1,121.75) ;
\draw [shift={(537.86,120.79)}, rotate = 511.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da40090887344122583] 
\draw    (517.86,108.21) -- (536.16,119.72) ;
\draw [shift={(537.86,120.79)}, rotate = 212.15] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44148920051151874] 
\draw    (558.71,120.21) -- (576.14,120.21) ;
\draw [shift={(578.14,120.21)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp8281008655924245] 
\draw  [draw opacity=0] (578.14,110.21) -- (618.29,110.21) -- (618.29,130.57) -- (578.14,130.57) -- cycle ; \draw   (578.14,110.21) -- (578.14,130.57)(588.14,110.21) -- (588.14,130.57)(598.14,110.21) -- (598.14,130.57)(608.14,110.21) -- (608.14,130.57)(618.14,110.21) -- (618.14,130.57) ; \draw   (578.14,110.21) -- (618.29,110.21)(578.14,120.21) -- (618.29,120.21)(578.14,130.21) -- (618.29,130.21) ; \draw    ;
%Rounded Rect [id:dp5344269055497854] 
\draw   (218,27.43) .. controls (218,23.01) and (221.58,19.43) .. (226,19.43) -- (250.71,19.43) .. controls (255.13,19.43) and (258.71,23.01) .. (258.71,27.43) -- (258.71,51.43) .. controls (258.71,55.85) and (255.13,59.43) .. (250.71,59.43) -- (226,59.43) .. controls (221.58,59.43) and (218,55.85) .. (218,51.43) -- cycle ;
%Straight Lines [id:da9973828070780348] 
\draw    (120.86,39.5) -- (216.14,39.5) ;
\draw [shift={(218.14,39.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3411365444456085] 
\draw    (258.86,39) -- (418.14,39.5) ;
%Straight Lines [id:da5701997367736331] 
\draw    (297.4,80.9) -- (297.81,98.79) ;
\draw [shift={(297.86,100.79)}, rotate = 268.68] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da245879419682548] 
\draw    (418.4,79.9) -- (418.04,98.5) ;
\draw [shift={(418,100.5)}, rotate = 271.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8264822410606818] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (129.86,42.72) .. controls (129.86,25.15) and (144.1,10.9) .. (161.68,10.9) -- (532.18,10.9) .. controls (549.75,10.9) and (564,25.15) .. (564,42.72) -- (564,138.18) .. controls (564,155.75) and (549.75,170) .. (532.18,170) -- (161.68,170) .. controls (144.1,170) and (129.86,155.75) .. (129.86,138.18) -- cycle ;
%Straight Lines [id:da8159210537128676] 
\draw    (297.4,39.7) -- (297.4,58.9) ;
\draw [shift={(297.4,60.9)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp8261426568953048] 
\draw  [draw opacity=0] (277.4,60.9) -- (317.54,60.9) -- (317.54,81.26) -- (277.4,81.26) -- cycle ; \draw   (277.4,60.9) -- (277.4,81.26)(287.4,60.9) -- (287.4,81.26)(297.4,60.9) -- (297.4,81.26)(307.4,60.9) -- (307.4,81.26)(317.4,60.9) -- (317.4,81.26) ; \draw   (277.4,60.9) -- (317.54,60.9)(277.4,70.9) -- (317.54,70.9)(277.4,80.9) -- (317.54,80.9) ; \draw    ;
%Shape: Grid [id:dp42560627641027393] 
\draw  [draw opacity=0] (398.4,59.9) -- (438.54,59.9) -- (438.54,80.26) -- (398.4,80.26) -- cycle ; \draw   (398.4,59.9) -- (398.4,80.26)(408.4,59.9) -- (408.4,80.26)(418.4,59.9) -- (418.4,80.26)(428.4,59.9) -- (428.4,80.26)(438.4,59.9) -- (438.4,80.26) ; \draw   (398.4,59.9) -- (438.54,59.9)(398.4,69.9) -- (438.54,69.9)(398.4,79.9) -- (438.54,79.9) ; \draw    ;
%Straight Lines [id:da31662051328483676] 
\draw    (418.14,39.5) -- (418.37,57.9) ;
\draw [shift={(418.4,59.9)}, rotate = 269.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Grid [id:dp28428263898063655] INPUT h
\draw  [draw opacity=0] (80,69.64) -- (120.14,69.64) -- (120.14,90) -- (80,90) -- cycle ; \draw   (80,69.64) -- (80,90)(90,69.64) -- (90,90)(100,69.64) -- (100,90)(110,69.64) -- (110,90)(120,69.64) -- (120,90) ; \draw   (80,69.64) -- (120.14,69.64)(80,79.64) -- (120.14,79.64)(80,89.64) -- (120.14,89.64) ; \draw    ;
%Straight Lines [id:da14826808759935606] 
\draw    (180,80) -- (180,98) ;
\draw [shift={(180,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2515630322243856] 
\draw    (120,79.64) -- (180,80) ;


% Text Node
\draw (168,114) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny Init}};
% Text Node
\draw (282,114) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Col QR};
% Text Node
\draw (400,114) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Diag QR};
% Text Node
\draw (63,114) node [anchor=north west][inner sep=0.75pt]    {$iv$};
% Text Node
\draw (63,31) node [anchor=north west][inner sep=0.75pt]    {$d$};
% Text Node INPUT h
\draw (63,72) node [anchor=north west][inner sep=0.75pt]    {$h$};
% Text Node
\draw (222,31) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny Perm(i)}};
% Text Node
% \draw (277.4,63.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{0}}$};
% % Text Node
% \draw (287.2,63.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{1}}$};
% % Text Node
% \draw (297.4,63.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{2}}$};
% % Text Node
% \draw (307.2,63.2) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{3}}$};
% % Text Node
% \draw (277.4,73.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{4}}$};
% % Text Node
% \draw (287.2,73.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{5}}$};
% % Text Node
% \draw (297.4,73.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{6}}$};
% % Text Node
% \draw (307.2,73.2) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{7}}$};
% % Text Node
% \draw (398.4,62.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{8}}$};
% % Text Node
% \draw (408.2,62.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{9}}$};
% % Text Node
% \draw (418.4,62.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{10}}$};
% % Text Node
% \draw (428.2,62.2) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{11}}$};
% % Text Node
% \draw (398.4,72.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{12}}$};
% % Text Node
% \draw (408.2,72.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{13}}$};
% % Text Node
% \draw (418.4,72.3) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{14}}$};
% % Text Node
% \draw (428.2,72.2) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.38em}{0.46em}\selectfont]  {$d_{s^{( i)}_{15}}$};
% Text Node
\draw (298,152.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$i=0,\dotsc ,\rho-1$};
% Text Node
\draw (594,89.4) node [anchor=north west][inner sep=0.75pt]    {$h$};
% Text Node
\draw (227,79.4) node [anchor=north west][inner sep=0.75pt]    {$v^{( i)}$};
% Text Node
\draw (480,77.4) node [anchor=north west][inner sep=0.75pt]    {$v^{(\rho-1)}$};
% Text Node
\draw (280,0) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny Blake2 compression function $F$}};
\end{tikzpicture}


==> figures/sponge_with_4x4_block_one_message_block.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,123); %set diagram left start at 0, and has height of 123

%Shape: Rectangle [id:dp8433803538862741] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (380.02,20.4) -- (410.13,20.4) -- (410.13,50.66) -- (380.02,50.66) -- cycle ;
%Shape: Rectangle [id:dp014493843046666566] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (280,20.24) -- (310.11,20.24) -- (310.11,50.5) -- (280,50.5) -- cycle ;
%Shape: Rectangle [id:dp9259884055493455] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (270,70.2) -- (270.02,100.1) -- (260.02,100.1) -- (260,70.21) -- cycle ;
%Shape: Rectangle [id:dp010781118907600584] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (230.02,100.2) -- (270.02,100.2) -- (270.02,110.2) -- (230.02,110.2) -- cycle ;
%Shape: Ellipse [id:dp1634740410998925] 
\draw   (294.86,90.19) .. controls (294.86,87.44) and (297.08,85.21) .. (299.8,85.21) .. controls (302.53,85.21) and (304.75,87.44) .. (304.75,90.19) .. controls (304.75,92.95) and (302.53,95.18) .. (299.8,95.18) .. controls (297.08,95.18) and (294.86,92.95) .. (294.86,90.19) -- cycle ;
%Straight Lines [id:da6710152233890574] 
\draw    (299.8,85.46) -- (299.8,95.18) ;
%Straight Lines [id:da43514468960306885] 
\draw    (294.86,90.19) -- (304.75,90.19) ;
%Straight Lines [id:da4365903716433732] 
\draw    (300.11,60.24) -- (299.83,83.21) ;
\draw [shift={(299.8,85.21)}, rotate = 270.71] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4080891606157835] 
\draw    (270.38,89.88) -- (292.53,90.17) ;
\draw [shift={(294.53,90.19)}, rotate = 180.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4458948138476999] 
\draw    (304.41,90.19) -- (327.12,90.08) ;
\draw [shift={(329.12,90.07)}, rotate = 539.71] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp6113932309444663] 
\draw   (329.37,76.44) .. controls (329.37,72.96) and (332.19,70.14) .. (335.67,70.14) -- (354.58,70.14) .. controls (358.07,70.14) and (360.89,72.96) .. (360.89,76.44) -- (360.89,103.45) .. controls (360.89,106.93) and (358.07,109.75) .. (354.58,109.75) -- (335.67,109.75) .. controls (332.19,109.75) and (329.37,106.93) .. (329.37,103.45) -- cycle ;
%Straight Lines [id:da7175058586507075] 
\draw    (360.82,90) -- (378.02,90) ;
\draw [shift={(380.02,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da09637279392728981] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (365.62,20.4) -- (365.62,120.8) ;
%Straight Lines [id:da6228956196351305] 
\draw    (395.76,70.16) -- (395.64,53.2) ;
\draw [shift={(395.62,51.2)}, rotate = 449.58] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Grid [id:dp9461389252018562] 
\draw  [draw opacity=0] (230.02,70.2) -- (270.02,70.2) -- (270.02,110.2) -- (230.02,110.2) -- cycle ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (240.02,70.2) -- (240.02,110.2)(250.02,70.2) -- (250.02,110.2)(260.02,70.2) -- (260.02,110.2) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (230.02,80.2) -- (270.02,80.2)(230.02,90.2) -- (270.02,90.2)(230.02,100.2) -- (270.02,100.2) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (230.02,70.2) -- (270.02,70.2) -- (270.02,110.2) -- (230.02,110.2) -- cycle ;
%Shape: Grid [id:dp7727475353661855] 
\draw  [draw opacity=0] (280.11,20.24) -- (320.11,20.24) -- (320.11,60.24) -- (280.11,60.24) -- cycle ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (290.11,20.24) -- (290.11,60.24)(300.11,20.24) -- (300.11,60.24)(310.11,20.24) -- (310.11,60.24) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (280.11,30.24) -- (320.11,30.24)(280.11,40.24) -- (320.11,40.24)(280.11,50.24) -- (320.11,50.24) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (280.11,20.24) -- (320.11,20.24) -- (320.11,60.24) -- (280.11,60.24) -- cycle ;
%Shape: Rectangle [id:dp2676394074304389] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (380.6,69.84) -- (410.71,69.84) -- (410.71,100.1) -- (380.6,100.1) -- cycle ;
%Shape: Grid [id:dp10112988200445683] 
\draw  [draw opacity=0] (380.71,69.84) -- (420.71,69.84) -- (420.71,109.84) -- (380.71,109.84) -- cycle ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (390.71,69.84) -- (390.71,109.84)(400.71,69.84) -- (400.71,109.84)(410.71,69.84) -- (410.71,109.84) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (380.71,79.84) -- (420.71,79.84)(380.71,89.84) -- (420.71,89.84)(380.71,99.84) -- (420.71,99.84) ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (380.71,69.84) -- (420.71,69.84) -- (420.71,109.84) -- (380.71,109.84) -- cycle ;
%Shape: Grid [id:dp6160542921700045] 
\draw  [draw opacity=0] (380.02,20.4) -- (410.22,20.4) -- (410.22,50.9) -- (380.02,50.9) -- cycle ; \draw   (380.02,20.4) -- (380.02,50.9)(390.02,20.4) -- (390.02,50.9)(400.02,20.4) -- (400.02,50.9)(410.02,20.4) -- (410.02,50.9) ; \draw   (380.02,20.4) -- (410.22,20.4)(380.02,30.4) -- (410.22,30.4)(380.02,40.4) -- (410.22,40.4)(380.02,50.4) -- (410.22,50.4) ; \draw    ;

% Text Node
\draw (280.56,22.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (290.22,22) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (300.22,22.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (280.56,31.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (290.22,32.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (300.22,31.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (280.56,41.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (290.22,42.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (300.22,41.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {m};
% Text Node
\draw (262.22,72.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (262.02,82.2) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (262.22,92.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (262.02,102.2) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (251.69,101.53) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (242.36,102.2) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (232.02,101.53) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {p};
% Text Node
\draw (337.89,83.73) node [anchor=north west][inner sep=0.75pt]    {$\Pi $};
% Text Node
\draw (293.67,3.07) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$m$};
% Text Node
\draw (389.78,3.07) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$h$};
% Text Node
\draw (311.4,22) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (311.46,32.65) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (310.96,42.9) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (311.21,52.29) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (301.21,52.29) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (290.96,52.29) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (282.21,52.04) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (250.71,72.79) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (241.46,72.79) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (232.02,72.6) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (250.71,82.54) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (241.46,82.54) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (232.02,82.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (250.96,92.54) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (241.71,92.54) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};
% Text Node
\draw (232.27,92.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$0$};


\end{tikzpicture}


==> fse-latex-class/settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.13154/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother


==> fse-latex-class/settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.13154/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

